PBPO: Prefix-Block Policy Optimization for Diffusion Language Models

Diffusion Large Language Models (dLLMs) commonly decode responses by proceeding autoregressively across blocks while iteratively denoising multiple tokens within each block. This structure makes block-level policy optimization a natural adaptation of autoregressive policy optimization. However, the exact likelihood of a completed block is intractable because it marginalizes over the intermediate states and reveal orders of the denoising process. To realize the block-level formulation, we construct a prefix-block state and use a single model evaluation to define a factorized one-step surrogate for the block likelihood. The resulting block surrogate ratio is a product of its token surrogate ratios, allowing variation at individual positions to propagate across the entire block before clipping. We therefore introduce Prefix-Block Policy Optimization (PBPO), which preserves block-level conditioning but applies surrogate importance weighting and clipping separately to each token. PBPO further diversifies repeated updates by resampling corrupted views of the prompt and revealed prefix, a design motivated by masked-dLLM pre-training. Under our analysis assumptions, block-product weighting amplifies the variance of gradient contributions relative to token-local weighting. Across two LLaDA-family initializations, six benchmarks, and three generation lengths, PBPO achieves competitive performance against existing dLLM RL methods.

==> tables/code_exp.tex <==
\begin{table}[t]
\centering
\caption{Main results across two coding benchmarks at generation lengths 128, 256, and 512.
Best result per column within each backbone block is in \textbf{bold}, and the second-best is \underline{underlined}.}
\label{tab:code_exp}
\small
\setlength{\tabcolsep}{4pt}
\resizebox{0.5\linewidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{3}{c}{\textbf{HumanEval}}
& \multicolumn{3}{c}{\textbf{MBPP}} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
\textbf{Baseline / Seq Len}
& \textbf{128} & \textbf{256} & \textbf{512}
& \textbf{128} & \textbf{256} & \textbf{512} \\
\midrule
\textit{LLaDA-8B-Instruct}
    & 23.17 & 31.71 & 30.49
    & 35.41 & 39.69 & 40.86 \\
\hspace{1em} d1
    & \underline{29.88} & 35.37 & \textbf{37.80}
    & 41.25 & 42.41 & 41.63 \\
\hspace{1em} wd1
    & 27.44 & 34.15 & \underline{37.20}
    & 42.80 & 42.02 & 42.80 \\
\hspace{1em} GDPO
    & 23.17 & \textbf{37.20} & 36.59
    & 42.41 & 41.25 & 42.80 \\
\hspace{1em} DMPO
    & 24.39 & \underline{35.98} & \textbf{37.80}
    & \underline{43.19} & \underline{43.58} & \underline{43.58} \\
\rowcolor[HTML]{F0F8FF}[\tabcolsep][\tabcolsep]
\rule[-0.85ex]{0pt}{3.1ex}\hspace{1em} \textbf{PBPO (Ours)}
    & \textbf{30.49} & \textbf{37.20} & \textbf{37.80}
    & \textbf{43.97} & \textbf{48.25} & \textbf{47.47} \\
\midrule
\textit{LLaDA-1.5}
    & 21.95 & 30.49 & 34.76
    & 36.19 & 44.36 & 38.91 \\
\hspace{1em} d1
    & \underline{26.22} & 33.54 & 33.54
    & 40.86 & \textbf{46.69} & 42.02 \\
\hspace{1em} wd1
    & 23.78 & 35.98 & 31.71
    & 40.08 & 40.47 & 42.41 \\
\hspace{1em} GDPO
    & 23.78 & 36.59 & \textbf{35.98}
    & 38.91 & \underline{45.91} & 41.25 \\
\hspace{1em} DMPO
    & 25.00 & \underline{39.63} & \underline{35.37}
    & \underline{42.41} & 44.36 & \underline{43.19} \\
\rowcolor[HTML]{F0F8FF}[\tabcolsep][\tabcolsep]
\rule[-0.85ex]{0pt}{3.1ex}\hspace{1em} \textbf{PBPO (Ours)}
    & \textbf{31.71} & \textbf{41.46} & \textbf{35.98}
    & \textbf{42.80} & \textbf{46.69} & \textbf{44.36} \\
\bottomrule
\end{tabular}%
}
\end{table}


==> tables/countdown_sudoku_exp.tex <==
\begin{wraptable}{r}
{0.5\textwidth}
\vspace{-10mm}
    \centering
    \caption{Main results across Countdown and Sudoku at generation lengths 128,
    256, and 512. Best result per column within each backbone block is in
    \textbf{bold}, and the second-best is \underline{underlined}.}
    \label{tab:countdown_sudoku_exp}

    \small
    \setlength{\tabcolsep}{4pt}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lcccccc}
    \toprule
    & \multicolumn{3}{c}{\textbf{Countdown}}
    & \multicolumn{3}{c}{\textbf{Sudoku}} \\
    \cmidrule(lr){2-4}
    \cmidrule(lr){5-7}
    \textbf{Baseline / Seq Len}
    & \textbf{128} & \textbf{256} & \textbf{512}
    & \textbf{128} & \textbf{256} & \textbf{512} \\
    \midrule
    \textit{LLaDA-8B-Instruct}
        & 19.92 & 17.97 & 17.97
        & 9.33 & 5.74 & 5.12 \\
    \hspace{1em} d1
        & 30.08 & 23.44 & 30.08
        & 21.29 & 14.98 & 9.76 \\
    \hspace{1em} wd1
        & 48.83 & 51.17 & 49.22
        & 24.40 & 24.16 & 22.97 \\
    \hspace{1em} GDPO
        & \textbf{62.50} & \textbf{73.05} & \textbf{73.05}
        & \underline{28.09} & \underline{28.09} & \underline{26.12} \\
    \hspace{1em} DMPO
        & 50.00 & 57.81 & \underline{64.84}
        & 21.15 & 17.13 & 15.50 \\
    \rowcolor[HTML]{F0F8FF}[\tabcolsep][\tabcolsep]
    \rule[-0.85ex]{0pt}{3.1ex}\hspace{1em} \textbf{PBPO (Ours)}
        & \underline{52.73} & \underline{64.06} & 64.45
        & \textbf{34.93} & \textbf{38.13} & \textbf{38.13} \\
    \midrule
    \textit{LLaDA-1.5}
        & 21.09 & 18.36 & 21.09
        & 13.78 & 10.10 & 8.33 \\
    \hspace{1em} d1
        & 29.69 & 19.14 & 33.20
        & 21.05 & 15.69 & 11.53 \\
    \hspace{1em} wd1
        & 42.97 & 56.25 & 48.05
        & 24.31 & 23.16 & 22.73 \\
    \hspace{1em} GDPO
        & \underline{51.56} & \underline{67.58} & \textbf{71.88}
        & 25.50 & \underline{26.70} & \underline{24.26} \\
    \hspace{1em} DMPO
        & 49.61 & 58.98 & \underline{69.92}
        & \underline{26.12} & 24.98 & 23.88 \\
    \rowcolor[HTML]{F0F8FF}[\tabcolsep][\tabcolsep]
    \rule[-0.85ex]{0pt}{3.1ex}\hspace{1em} \textbf{PBPO (Ours)}
        & \textbf{57.03} & \textbf{69.14} & 69.53
        & \textbf{37.75} & \textbf{39.33} & \textbf{36.17} \\
    \bottomrule
    \end{tabular}%
    }
    \vspace{-5mm}
\end{wraptable}

==> tables/vertial_main_exp.tex <==
\begin{table}[t]
\centering
\caption{Main results across six reasoning and coding benchmarks at generation lengths 128, 256, and 512.
Best result per row within each backbone block is in \textbf{bold}, and the second-best is \underline{underlined}. \kt{On Sudoku, increasing generation length reduces base-model accuracy for both backbones, suggesting that longer diffusion trajectories may amplify decoding errors rather than improve solution quality.}}
\label{tab:vertical_main_exp}
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.95}
\begin{tabular}{llccccc>{\columncolor[HTML]{F0F8FF}}c}
\toprule
\textbf{Dataset} & \textbf{Seq Len} & \textbf{Base} & \textbf{d1} & \textbf{wd1} & \textbf{GDPO} & \textbf{DMPO} & \textbf{PBPO (Ours)} \\
\midrule
\multicolumn{8}{l}{\textit{LLaDA-8B-Instruct}} \\
\midrule
\textbf{GSM8K} & \textbf{128} & 69.37 & 72.55 & 73.01 & \underline{75.66} & 75.59 & \textbf{76.72} \\
\textbf{GSM8K} & \textbf{256} & 77.94 & 78.01 & 80.06 & 79.91 & \underline{80.74} & \textbf{84.08} \\
\textbf{GSM8K} & \textbf{512} & 79.61 & 81.20 & 81.50 & 80.59 & \underline{82.79} & \textbf{84.38} \\
\addlinespace
\textbf{MATH500} & \textbf{128} & 26.80 & 29.00 & \underline{32.80} & 31.40 & 29.80 & \textbf{34.80} \\
\textbf{MATH500} & \textbf{256} & 32.80 & 34.40 & 34.80 & 34.80 & \underline{35.40} & \textbf{36.80} \\
\textbf{MATH500} & \textbf{512} & 34.20 & 37.60 & 36.20 & 37.40 & \underline{38.20} & \textbf{41.40} \\
\addlinespace
\textbf{HumanEval} & \textbf{128} & 23.17 & \underline{29.88} & 27.44 & 23.17 & 24.39 & \textbf{30.49} \\
\textbf{HumanEval} & \textbf{256} & 31.71 & 35.37 & 34.15 & \textbf{37.20} & \underline{35.98} & \textbf{37.20} \\
\textbf{HumanEval} & \textbf{512} & 30.49 & \textbf{37.80} & \underline{37.20} & 36.59 & \textbf{37.80} & \textbf{37.80} \\
\addlinespace
\textbf{MBPP} & \textbf{128} & 35.41 & 41.25 & 42.80 & 42.41 & \underline{43.19} & \textbf{43.97} \\
\textbf{MBPP} & \textbf{256} & 39.69 & 42.41 & 42.02 & 41.25 & \underline{43.58} & \textbf{48.25} \\
\textbf{MBPP} & \textbf{512} & 40.86 & 41.63 & 42.80 & 42.80 & \underline{43.58} & \textbf{47.47} \\
\addlinespace
\textbf{Countdown} & \textbf{128} & 19.92 & 30.08 & 48.83 & \textbf{62.50} & 50.00 & \underline{52.73} \\
\textbf{Countdown} & \textbf{256} & 17.97 & 23.44 & 51.17 & \textbf{73.05} & 57.81 & \underline{64.06} \\
\textbf{Countdown} & \textbf{512} & 17.97 & 30.08 & 49.22 & \textbf{73.05} & \underline{64.84} & 64.45 \\
\addlinespace
\textbf{Sudoku} & \textbf{128} & 9.33 & 21.29 & 24.40 & \underline{28.09} & 21.15 & \textbf{34.93} \\
\textbf{Sudoku} & \textbf{256} & 5.74 & 14.98 & 24.16 & \underline{28.09} & 17.13 & \textbf{38.13} \\
\textbf{Sudoku} & \textbf{512} & 5.12 & 9.76 & 22.97 & \underline{26.12} & 15.50 & \textbf{38.13} \\
\midrule
\multicolumn{8}{l}{\textit{LLaDA-1.5}} \\
\midrule
\textbf{GSM8K} & \textbf{128} & 71.27 & 74.15 & 73.09 & \underline{74.60} & 49.81 & \textbf{78.24} \\
\textbf{GSM8K} & \textbf{256} & 79.38 & \underline{81.35} & 78.77 & 78.39 & 50.87 & \textbf{83.47} \\
\textbf{GSM8K} & \textbf{512} & \underline{82.11} & 80.74 & 81.12 & 79.38 & 51.33 & \textbf{84.61} \\
\addlinespace
\textbf{MATH500} & \textbf{128} & 28.40 & 28.00 & 30.00 & 30.20 & \underline{31.40} & \textbf{33.40} \\
\textbf{MATH500} & \textbf{256} & 32.20 & \underline{36.20} & 34.80 & 34.40 & 35.80 & \textbf{42.00} \\
\textbf{MATH500} & \textbf{512} & \underline{38.40} & 36.00 & 36.40 & \underline{38.40} & \textbf{39.00} & \textbf{39.00} \\
\addlinespace
\textbf{HumanEval} & \textbf{128} & 21.95 & \underline{26.22} & 23.78 & 23.78 & 25.00 & \textbf{31.71} \\
\textbf{HumanEval} & \textbf{256} & 30.49 & 33.54 & 35.98 & 36.59 & \underline{39.63} & \textbf{41.46} \\
\textbf{HumanEval} & \textbf{512} & 34.76 & 33.54 & 31.71 & \textbf{35.98} & \underline{35.37} & \textbf{35.98} \\
\addlinespace
\textbf{MBPP} & \textbf{128} & 36.19 & 40.86 & 40.08 & 38.91 & \underline{42.41} & \textbf{42.80} \\
\textbf{MBPP} & \textbf{256} & 44.36 & \textbf{46.69} & 40.47 & \underline{45.91} & 44.36 & \textbf{46.69} \\
\textbf{MBPP} & \textbf{512} & 38.91 & 42.02 & 42.41 & 41.25 & \underline{43.19} & \textbf{44.36} \\
\addlinespace
\textbf{Countdown} & \textbf{128} & 21.09 & 29.69 & 42.97 & \underline{51.56} & 49.61 & \textbf{57.03} \\
\textbf{Countdown} & \textbf{256} & 18.36 & 19.14 & 56.25 & \underline{67.58} & 58.98 & \textbf{69.14} \\
\textbf{Countdown} & \textbf{512} & 21.09 & 33.20 & 48.05 & \textbf{71.88} & \underline{69.92} & 69.53 \\
\addlinespace
\textbf{Sudoku} & \textbf{128} & 13.78 & 21.05 & 24.31 & 25.50 & \underline{26.12} & \textbf{37.75} \\
\textbf{Sudoku} & \textbf{256} & 10.10 & 15.69 & 23.16 & \underline{26.70} & 24.98 & \textbf{39.33} \\
\textbf{Sudoku} & \textbf{512} & 8.33 & 11.53 & 22.73 & \underline{24.26} & 23.88 & \textbf{36.17} \\
\bottomrule
\end{tabular}
\end{table}

